Constrained intersection representations and forbidden patterns

We study the interplay between two types of graph classes: the ones defined by intersections of geometric objects and the ones defined by the absence of a substructure. More precisely, we study intersection graphs that are grounded, that is, the objects lie above a horizontal line that they touch, and ordered graphs with forbidden patterns, that is, ordered graphs that avoid a set of ordered induced subgraphs. These two approaches are fundamentally different, but it is known that several interesting graph classes have both types of characterizations, and we aim to understand whether this is a general phenomenon. Our contributions are the following. First, we identify a family of patterns on four vertices and a natural hierarchy of intersection graphs of strings whose classes are nicely interleaved. This raises hopes to prove connections between the two perspectives. Second, we dampen these hopes by proving that a class of (ordered) intersection graphs that we study cannot be characterized by a finite set of forbidden patterns. Third, we show a dual impossibility result: there exists a pattern-defined class of our hierarchy that admits no intersection representation, if we require this representation to be closed under natural operations such as translation and scaling. However, it turns out that if we allow slightly more exotic intersection representations, then we can find one for this pattern-defined class.

==> intro-diagram/Pa.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> intro-diagram/Pab.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> intro-diagram/Pb.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> intro-diagram/interval.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw (a) to[bend left=50] (c);
			\draw[dashed] (a) to (b);
		\end{tikzpicture}

==> rounding-rectangle-trick.tex <==
\makeatletter

\pgfkeys{/pgf/.cd,
 rectangle corner radius/.initial=3pt
}
\newif\ifpgf@rectanglewrc@donecorner@
\def\pgf@rectanglewithroundedcorners@docorner#1#2#3#4{%
  \edef\pgf@marshal{%
    \noexpand\pgfintersectionofpaths
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
        \noexpand\pgfpathlineto{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
      }%
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpointadd
          {\noexpand\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}%
          {\noexpand\pgfpoint{#1}{#2}}}%
        \noexpand\pgfpatharc{#3}{#4}{\cornerradius}%
      }%
    }%
  \pgf@process{\pgf@marshal\pgfpointintersectionsolution{1}}%
  \pgf@process{\pgftransforminvert\pgfpointtransformed{}}%
  \pgf@rectanglewrc@donecorner@true
}
\pgfdeclareshape{rectangle with rounded corners}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}

  \savedmacro\cornerradius{%
    \edef\cornerradius{\pgfkeysvalueof{/pgf/rectangle corner radius}}%
  }

  \backgroundpath{%
    \northeast\advance\pgf@y-\cornerradius\relax
    \pgfpathmoveto{}%
    \pgfpatharc{0}{90}{\cornerradius}%
    \northeast\pgf@ya=\pgf@y\southwest\advance\pgf@x\cornerradius\relax\pgf@y=\pgf@ya
    \pgfpathlineto{}%
    \pgfpatharc{90}{180}{\cornerradius}%
    \southwest\advance\pgf@y\cornerradius\relax
    \pgfpathlineto{}%
    \pgfpatharc{180}{270}{\cornerradius}%
    \northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradius\southwest\pgf@x=\pgf@xa
    \pgfpathlineto{}%
    \pgfpatharc{270}{360}{\cornerradius}%
    \northeast\advance\pgf@y-\cornerradius\relax
    \pgfpathlineto{}%
  }

  \anchor{before north east}{\northeast\advance\pgf@y-\cornerradius}
  \anchor{after north east}{\northeast\advance\pgf@x-\cornerradius}
  \anchor{before north west}{\southwest\pgf@xa=\pgf@x\advance\pgf@xa\cornerradius
    \northeast\pgf@x=\pgf@xa}
  \anchor{after north west}{\northeast\pgf@ya=\pgf@y\advance\pgf@ya-\cornerradius
    \southwest\pgf@y=\pgf@ya}
  \anchor{before south west}{\southwest\advance\pgf@y\cornerradius}
  \anchor{after south west}{\southwest\advance\pgf@x\cornerradius}
  \anchor{before south east}{\northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradius
    \southwest\pgf@x=\pgf@xa}
  \anchor{after south east}{\southwest\pgf@ya=\pgf@y\advance\pgf@ya\cornerradius
    \northeast\pgf@y=\pgf@ya}

  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa% 
    \advance\pgf@y by\pgf@ya%
    \pgfextract@process\borderpoint{}%
    %
    \pgf@rectanglewrc@donecorner@false
    %
    % do southwest corner
    \southwest\pgf@xc=\pgf@x\pgf@yc=\pgf@y
    \advance\pgf@xc\cornerradius\relax\advance\pgf@yc\cornerradius\relax 
    \borderpoint
    \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
      \pgf@rectanglewithroundedcorners@docorner{-\cornerradius}{0pt}{180}{270}%
    \fi\fi
    %
    % do southeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \southwest\pgf@yc=\pgf@y\relax\northeast\pgf@xc=\pgf@x\relax
      \advance\pgf@xc-\cornerradius\relax\advance\pgf@yc\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{-\cornerradius}{270}{360}%
      \fi\fi
    \fi
    %
    % do northeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@xc=\pgf@x\relax\pgf@yc=\pgf@y\relax
      \advance\pgf@xc-\cornerradius\relax\advance\pgf@yc-\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{\cornerradius}{0pt}{0}{90}%
      \fi\fi
    \fi
    %
    % do northwest corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@yc=\pgf@y\relax\southwest\pgf@xc=\pgf@x\relax
      \advance\pgf@xc\cornerradius\relax\advance\pgf@yc-\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{\cornerradius}{90}{180}%
      \fi\fi
    \fi
  }
}

\makeatother

%\begin{tikzpicture}
%  \draw node(rc)[
%    rectangle with rounded corners,draw,rectangle corner radius=10pt,align=center]
%    {\large rectangle with rounded corners\\\large rectangle with rounded corners\\\large rectangle with rounded corners};
%  \fill[red,every node/.style={font=\tiny}]
%        \foreach \d/\p in {before north east/right,after north east/above,
%                           before north west/above,after north west/left,
%                           before south west/left,after south west/below,
%                           before south east/right,after south east/right}
%                       { (rc.\d) circle(1pt) node[\p]{\d} };
%  \draw[blue,draw opacity=0.3]\foreach\a in {0,...,360} {(rc)--+(\a:5cm)};
%\end{tikzpicture}
%
%\end{document}

==> strict-inclusions-diagram/P0.tex <==
\begin{tikzpicture}   
[scale=0.8,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {};   
\node (n2) at (1,0) {};   
\node (n3) at (2,0)  {};   
\node (n4) at (3,0)  {};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4);
 
\end{tikzpicture}

==> strict-inclusions-diagram/Pa.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> strict-inclusions-diagram/Pab.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> strict-inclusions-diagram/Pb.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}
